Informed Pooled Testing with Quantitative Assays

Pooled testing is widely used for screening for viral or bacterial infections with low prevalence when individual testing is not cost-efficient. Pooled testing with qualitative assays that give binary results has been well-studied. However, characteristics of pooling with quantitative assays were mostly demonstrated using simulations or empirical studies. We investigate properties of three pooling strategies with quantitative assays: traditional two-stage mini-pooling (MP) (Dorfman, 1943), mini-pooling with deconvolution algorithm (MPA) (May et al., 2010), and marker-assisted MPA (mMPA) (Liu et al., 2017). MPA and mMPA test individuals in a sequence after a positive pool and implement a deconvolution algorithm to determine when testing can cease to ascertain all individual statuses. mMPA uses information from other available markers to determine an optimal order for individual testings. We derive and compare the general statistical properties of the three pooling methods. We show that with a proper pool size, MP, MPA, and mMPA can be more cost-efficient than individual testing, and mMPA is superior to MPA and MP. For diagnostic accuracy, mMPA and MPA have higher specificity and positive predictive value but lower sensitivity and negative predictive value than MP and individual testing. Included in this paper are applications to various simulations and an application for HIV treatment monitoring.

==> Theorem3_A3_Proof.tex <==
\begin{proof}
The following will be an in-depth fleshed out and detailed proof of Theorem 3. Recall that
\[
M_{\mathrm{mMPA}}^{(a)} = 1 + \sum_{j=1}^{K-1}\mathbf{1}\{T_{[j]}^{(a)}>C\}
\]
where $T_{[j]}^{(a)} = \textstyle\sum_{l=j}^{K} V_{[l]}^{(a)}$.\\
\indent Then it follows by the additivity of expectation
\begin{align*}
\mathbb{E}(M_{\mathrm{mMPA}}^{(a)}) &
= \mathbb{E}(1+\sum_{j=1}^{K-1}\mathbf{1}\{T_{[j]}^{(a)}>C \}) \\
 & = 1 + \sum_{j=1}^{K-1} \mathbb{E}\mathbf{1}\{T_{[j]}^{(a)} > C\} \\
 & = 1 + \sum_{j=1}^{K-1}\Pr(T_{[j]}^{(a)}>C)\\
\end{align*}
Similarly, we have 
\[
M_{\mathrm{mMPA}}^{(b)} = 1 + \sum_{j=1}^{K-1}\mathbf{1}\{T_{[j]}^{(b)}>C\}
\]
where $T_{[j]}^{(b)} = \textstyle\sum_{l=j}^{K} V_{[l]}^{(b)}$. and\\
\begin{align*}
    \mathbb{E}(M_{\mathrm{mMPA}}^{(b)}) &
= \mathbb{E}(1+\sum_{j=1}^{K-1}\mathbf{1}\{T_{[j]}^{(b)}>C \}) \\
 & = 1 + \sum_{j=1}^{K-1} \mathbb{E}\mathbf{1}\{T_{[j]}^{(b)} > C\} \\
 & = 1 + \sum_{j=1}^{K-1}\Pr(T_{[j]}^{(b)}>C)\\
\end{align*}
Note 
\begin{align*}
    T_{[1]}^{(a)} &
    = \sum_{l = 1}^{K}V_{[l]}^{(a)}\\
    & = \sum_{l = 1}^{K}V_{l}^{(a)}\\
    & = \sum_{l = 1}^{K}V_{l}\\
\end{align*}
and for $j\ge2$
\begin{align*}
      T_{[1]}^{(a)} &
    = \sum_{l = 1}^{K}V_{[l]}^{(a)}\\
    & = \sum_{l = 1}^{K}V_{l}^{(a)} - \sum_{l = 1}^{j-1}V_{l}^{(a)}\\
    & = \sum_{l = 1}^{K}V_{l} - \sum_{l = 1}^{j-1}V_{l}^{(a)}\\
\end{align*}
Similarly, 
\begin{align*}
     T_{[1]}^{(b)} &
    = \sum_{l = 1}^{K}V_{[l]}^{(b)}\\
    & = \sum_{l = 1}^{K}V_{l}^{(b)}\\
    & = \sum_{l = 1}^{K}V_{l}\\
\end{align*}
and for $j\ge2$
\begin{align*}
      T_{[1]}^{(b)} &
    = \sum_{l = 1}^{K}V_{[l]}^{(b)}\\
    & = \sum_{l = 1}^{K}V_{l}^{(b)} - \sum_{l = 1}^{j-1}V_{l}^{(b)}\\
    & = \sum_{l = 1}^{K}V_{l} - \sum_{l = 1}^{j-1}V_{l}^{(b)}\\
\end{align*}
Obviously, $T_{[1]}^{(a)}=T_{[1]}^{(b)}$. Moreover, it is assumed that $S^{(a)}$ is a stronger risk score than $S^{(b)}$, namely,
\[
\sum_{l=1}^{j-1} V_{[l]}^{(a)} \succeq \sum_{l=1}^{j-1} V_{[l]}^{(a)},\quad 2\le j \le K.
\]

then for all non-decreasing functions $g$,
\[
\mathbb{E}g(\sum_{l=1}^{j-1}V_{[l]}^{(a)}) \ge \mathbb{E}g(\sum_{l=1}^{j-1}V_{[l]}^{(b)})
\]
In particular, for any fixed $A$, letting $g(x)=\mathbf{1}{x>A}$, we have
\[
\Pr(\sum_{l=1}^{j-1}V_{[l]}^{(a)} > A) \ge \Pr(\sum_{l=1}^{j-1}V_{[l]}^{(b)} > A) ,\quad 2\le j \le K
\]
and so equivalently,
\[
\Pr(\sum_{l=1}^{j-1}V_{[l]}^{(a)} \le A) \le \Pr(\sum_{l=1}^{j-1}V_{[l]}^{(b)} \le A) ,\quad 2\le j \le K
\]
In combination, it then follows
\[
\Pr(T_{[1]}^{(a)} > C) = \Pr(T_{[1]}^{(b)} > C) = \Pr(\sum_{l=1}^{K} V_{l} > C)
\]
and for $2\le j\le K$
\begin{align*}
    \Pr(T_{[1]}^{(a)} > C) &
    = \Pr(\sum_{l=1}^{K} V_{[l]} - \sum_{l=1}^{j-1} V_{[l]}^{(a)} > C)\\
    & = \Pr(\sum_{l=1}^{j-1} V_{[l]}^{(a)} < \sum_{l=1}^{K} V_{l} - C)\\
    & \leq \Pr(\sum_{l=1}^{j-1} V_{[l]}^{(b)} < \sum_{l=1}^{K} V_{l} - C)\\ 
    & = \Pr(T_{[j]}^{(b)} > C)\\ 
\end{align*}
where the inequality we have used the fact that for any $A$
\[
\Pr(\sum_{l=1}^{j-1}V_{[l]}^{(a)} \le A) \le \Pr(\sum_{l=1}^{j-1}V_{[l]}^{(b)} \le A) ,\quad 2\le j \le K
\]
Thus we have
\begin{align*}
  \mathbb{E}M_{\mathrm{mMPA}}^{(a)} &
  = 1 + \sum_{j=1}^{K-1} \Pr(T_{[j]}^{(a)} > C)\\
  & = 1 + \Pr(T_{[l]}^{(a)} > C) + \sum_{j=2}^{K-1} \Pr(T_{[j]}^{(a)} > C) \\
  & \leq 1 + \Pr(T_{[l]}^{(b)} > C) + \sum_{j=2}^{K-1} \Pr(T_{[j]}^{(b)} > C)\\
  & = \mathbb{E}M_{\mathrm{mMPA}}^{(b)}\\
\end{align*}
The proof is complete.
\end{proof}

==> name.tex <==
\subsection{Proof of of Theorem \ref{thm:The-diagnostic-accuracies}\label{appndx:diagnostic}}
\begin{proof}
We assume that $\varepsilon$ and $\varepsilon^{-1}$ have the same
distribution. We rewrite and denote the sensitivity of individual
testing as
\[
\mathrm{SENS}=\Pr(V>C\varepsilon|V>C).
\]
Note that in this equation both $V$ and $\varepsilon$ are random
variables. For MP, let us denote the measurement error testing the
pooled sample by $\varepsilon_{0}$ and the $k$th individual sample
by $\varepsilon_{k}.$ If we assume that the pool test and individual
test are independent, the probability of correctly classifying the
individual, given that the $k$th individual is experiencing ART failure,
is
\begin{align*}
\mathrm{SENS}_{\mathrm{MP}} & =\Pr\{T_{1}>C\varepsilon_{0}|V_{k}>C\}\Pr(V_{k}>C\varepsilon_{k}|V_{k}>C)\\
 & =\Pr\{V_{k}>C\varepsilon_{0}-(T_{1}-V_{k})|V_{k}>C\}\mathrm{\times SENS}\\
 & >\Pr\{V_{k}>C\varepsilon_{0}|V_{k}>C\}\times\mathrm{SENS}\\
 & =\mathrm{SENS}^{2},
\end{align*}
which means $\mathrm{SENS} ^ 2<\mathrm{SENS}_{\mathrm{MP}}<\mathrm{SENS}$.
Note that in reality $(T_{1}-V_{k})$ is often not small relatively
to the magnitude of the error $C(1-\varepsilon_{0})$. In this case
as $\Pr(T_{1}-V_{k}\ge C(1-\varepsilon_{0}))\rightarrow1$, $\Pr\{V_{1}>C\varepsilon_{0}|V_{k}>C\}\rightarrow1$
and $\mathrm{SENS}_{\mathrm{MP}}\rightarrow\mathrm{SENS}$. Further,
\begin{align*}
\mathrm{SENS}_{\mathrm{MPA}} & =\Pr\{T_{1}>C\varepsilon_{0}|V_{k}>C\}\Pr(\textrm{"all subpools test positive"})\Pr(V_{k}>C\varepsilon_{k}|V_{k}>C)\\
 & <\Pr\{T_{1}>C\varepsilon_{0}|V_{k}>C\}\Pr(V_{k}>C\varepsilon_{k}|V_{k}>C)=\mathrm{SENS}_{\mathrm{MP}}.
\end{align*}
Because mMPA requires a smaller number of tests in between, $\mathrm{SENS}_{\mathrm{mMPA}}>\mathrm{SENS}_{\mathrm{MPA}}$.
Summarizing these results, we have
\[
\mathrm{SENS}>\mathrm{SENS}_{\mathrm{MP}}>\mathrm{SENS}_{\mathrm{mMPA}}>\mathrm{SENS}_{\mathrm{MPA}}.
\]

Proof of the relationships in specificity among these testing procedures follows the same strategy as above.

Whitney: For PPV and NPV, can we prove similar relationships using the 


A5. Proof of Theorem 6.

{\bf Theorem 6}. Suppose that the same pool size is used for MP, MPA, and mMPA, and the marker used by mMPA is nontrivial. The diagnostic  accuracies of individual testing (IND), MP, MPA and mMPA have the following orders: for sensitivity and NPV,
$$
IND>MP>mMPA>MPA
$$
and for specificity and PPV
$$
 mMPA>MPA>MP>IND
$$
\end{proof}
\subsection{Proof of of Theorem 6 PPV}
\begin{proof}

\begin{align*}
\mathrm{PPV}_{\mathrm{POOL}} &
= \Pr(V_{k} > C | \textrm{"pooled testing classifies the sample as positive"}) \\
& = \frac{\Pr(V_{k}, \textrm{"pooled testing classifies the sample as positive"})} {\Pr(\textrm{"pooled testing classifies the sample as positive"})}
\end{align*}

\begin{align*}
\mathrm{PPV}_{\mathrm{IND}} &
= \frac{\Pr(V_{k} > C, \textrm{"IND test classifies the kth sample as positive"})} {\Pr(\textrm{"IND test classifies the kth sample as positive"})} \\
& = \frac{\Pr(V_{k}>C, V_{k}\varepsilon_{k}>C)}{\Pr(V_{k}\varepsilon_{k}>C)}\\
\end{align*}

\begin{align*}
\mathrm{PPV}_{\mathrm{MP}} &
= \frac{\Pr(V_{k} > C, \textrm{"MP test classifies the kth sample as positive"})} {\Pr(\textrm{"MP test classifies the kth sample as positive"})} \\
& = \frac{\Pr(T_{1}\eta_{1}>C, V_{k}\varepsilon_{k}>C, V_{k}>C)}   {\Pr(T_{1}\eta_{1}, V_{k}\varepsilon_{k}>C)}\\
\end{align*}

Thus,
\begin{align*}
   \mathrm{PPV}_{\mathrm{MP}} &
= \frac{\Pr(T_{1}\eta_{1}>C, V_{k}\varepsilon_{k}>C, V_{k}>C)}   {\Pr(T_{1}\eta_{1}, V_{k}\varepsilon_{k}>C)}\\
& = \frac{\Pr(T_{1}\eta_{1}>C |V_{k}\varepsilon_{k}>C, V_{k}>C) \Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)}                         {\Pr(T_{1}\eta_{1}>C|V_{k}\varepsilon_{k}>C) \Pr(V_{k}\varepsilon_{k}>C)}\\
& = \frac{\Pr(T_{1}\eta_{1}>C |V_{k}\varepsilon_{k}>C, V_{k}>C)}                         {\Pr(T_{1}\eta_{1}>C|V_{k}\varepsilon_{k}>C)} * \frac{\Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)}{\Pr(V_{k}\varepsilon_{k}>C)}\\
& = \frac{\Pr(T_{1}\eta_{1}>C |V_{k}\varepsilon_{k}>C, V_{k}>C)}                         {\Pr(T_{1}\eta_{1}>C|V_{k}\varepsilon_{k}>C)} * \mathrm{PPV}_{\mathrm{IND}} \\
\end{align*}
Because assuming 
\begin{equation}
\frac{\Pr(T_{1}\eta_{1}>C |V_{k}\varepsilon_{k}>C, V_{k}>C)}                         {\Pr(T_{1}\eta_{1}>C|V_{k}\varepsilon_{k}>C)}>1
\end{equation}
is reasonable, we have that $\mathrm{PPV}_{\mathrm{MP}} > \mathrm{PPV}_{\mathrm{IND}}$.

\begin{align*}
\mathrm{PPV}_{\mathrm{MPA}} &
= \frac{\Pr(V_{k} > C, \textrm{"MPA test classifies the kth sample as positive"})} {\Pr(\textrm{"MPA test classifies the kth sample as positive"})} \\
\end{align*}

The denominator is 

\begin{align*}
    \frac{1}{K} [\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})] &\\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}) & \\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+ V_{\pi_{2}}\varepsilon_{2}\eta_{2}+C\eta_{1}, V_{k}>C\varepsilon_{k})\\
    + \dots \\
\end{align*}

The denominator above we will call $B$. It can also be expressed more concisely in the form of:
\begin{align*}
   
\end{align*}

The numerator is:
\begin{align*}
   \frac{1}{K} [\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C) &\\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C) & \\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+ V_{\pi_{2}}\varepsilon_{2}\eta_{2}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)]\\
    + \dots \\ 
\end{align*}
The denominator above we will call $A$. It can also be expressed more concisely in the form of:

Then, we have that 
\[
\mathrm{PPV}_{\mathrm{MPA}} = \frac{A}{B}
\]
Next, we set out to compare $\mathrm{PPV}_{\mathrm{MPA}}$ and $\mathrm{PPV}_{\mathrm{MPA}}$. 

Our goal here then, is to provide a condition such that $\mathrm{PPV}_{\mathrm{MPA}} > \mathrm{PPV}_{\mathrm{MPA}}$
Namely,
\[ 
\frac{A}{B} > \frac{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}
\]

\[
\frac{A}{B} > \frac{C}{D} \Longleftrightarrow \frac{A}{B} > \frac{C}{D} 
\]

Therefore, we need to prove that
\[\frac{A}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)} > \frac{B}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}
\]

The factor $\frac{1}{K}$ cancels and therefore do not matter.

\begin{align*}
    \frac{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)} & \\ 
    + \frac{\Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)} & \\
    + \cdots
\end{align*}
is greater than
\begin{align*}
    \frac{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})} & \\
     + \frac{\Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k})} {\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}\\
    + \cdots
\end{align*}

Our simplest and most direct approach is to compare the two term by term, correspondingly. It is clearly evident that the individual term-by-term comparisons hold true, therefore we have that $\mathrm{PPV}_{\mathrm{MPA}}>\mathrm{PPV}_{\mathrm{MP}}.$

\begin{align*}
\mathrm{PPV}_{\mathrm{mMPA}} &
= \frac{\Pr(V_{k} > C, \textrm{"mMPA test classifies the kth sample as positive"})} {\Pr(\textrm{"mMPA test classifies the kth sample as positive"})} \\
\end{align*}

\begin{align*}
\mathrm{B_{m}} & \\
   =  \frac{1}{K} [\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}|\sigma_{1}=k) &\\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}|\sigma_{2}=k) & \\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+ V_{\pi_{2}}\varepsilon_{2}\eta_{2}+C\eta_{1}, V_{k}>C\varepsilon_{k}|\sigma_{3}=k)]\\
    + \dots \\ 
\end{align*}

\begin{align*}
    \mathrm{A_{m}} & \\
   =  \frac{1}{K} [\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{1}=k) &\\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{2}=k) & \\
    + \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+ V_{\pi_{2}}\varepsilon_{2}\eta_{2}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{3}=k)]\\
    + \dots \\ 
\end{align*}
We want to find a condition such that $\mathrm{PPV}_{\mathrm{mMPA}}>\mathrm{PPV}_{\mathrm{MP}}$.
Namely, 
\[
\frac{A_{m}}{B_{m}}>\frac{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)} {\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}
\]
Equivalently,
\[
\frac{A_{m}}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)} > \frac{B_{m}}{\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k})}
\]
Similar to the strategy used above, we can compare term-by-term. It is clearly evident that the individual term-by-term comparisons hold true, therefore we have that $\mathrm{PPV}_{\mathrm{mMPA}}>\mathrm{PPV}_{\mathrm{MP}}.$ 
It remains to show that $\mathrm{PPV}_{\mathrm{mMPA}}>\mathrm{PPV}_{\mathrm{MPA}}.$ 
\end{proof}

\subsection{Proof of of Theorem 6 Sensitivity}
\begin{proof}
Recall that 
\[
\mathrm{SENS}_{\mathrm{pool}} = \Pr(\textrm{"pool tests positive and the sample tests positive}|V_{k}>C)
\]
where the region of concern is $1\le k \le K$. $k$ denotes the $kth$ individual and $K$ is the size of the pool. 

$V_{k}$ stands for the true value of the kth individual. 
$V_{k}\varepsilon_{k}$ stands for the observed value where $\varepsilon_{k}$ is the measurement error.
\end{proof}

\begin{proof}
(1) Let's consider the Sensitivity of IND, MP, MPA, and mMPA.
\begin{align*}
    \mathrm{SENS}_{\mathrm{IND}} &
    = \Pr(V_{k}\varepsilon_{k}>C|V_{k}>C)\\
    & = \frac{\Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)}{\Pr(V_{k}>C)}\\
    & = \frac{\Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)}{\Pr(V_{k}>C)}\\
    & = \frac{\Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)}{\Pr(V_{k}>C)}\\
\end{align*}
Here, we use the fact that $\varepsilon$ and $\varepsilon^{-1}$ have the same
distribution. Additionally, we make use of the fact that $\varepsilon_{k}$ is independent of $V_{k}$s.
\begin{align*}
    \mathrm{SENS}_{\mathrm{MP}} &
    = \Pr(\textrm{"MP classifies the kth sample as positive"}|V_{k}>C)\\
    & = \frac{\Pr(\textrm{"MP classifies the kth sample as positive"}, V_{k}>C)}{\Pr(V_{k}>C)}\\
    & = \frac{\Pr(T_{1}\varepsilon_{0}>C,V_{k}\varepsilon_{k}>C, V_{k}>C)}{\Pr(V_{k}>C)}\\
    & = \frac{\Pr(T_{1}>C{\varepsilon_{0}}^{-1},V_{k}>C{\varepsilon_{k}}^{-1}, V_{k}>C)}{\Pr(V_{k}>C)}\\
    & = \frac{\Pr(T_{1}>C\varepsilon_{0},V_{k}>C\varepsilon_{k}, V_{k}>C)}{\Pr(V_{k}>C)}\\
\end{align*}
Since 
\[\Pr(T_{1}>C\varepsilon_{0},V_{k}>C\varepsilon_{k}, V_{k}>C)<\Pr(V_{k}\varepsilon_{k}>C, V_{k}>C)
\]
then, we have that $\mathrm{SENS}_{\mathrm{MP}}<\mathrm{SENS}_{\mathrm{IND}}$.

For $\mathrm{SENS}_{\mathrm{MPA}}$, we have that
\[
\mathrm{SENS}_{\mathrm{MPA}} = \frac{\Pr(\textrm{MPA classifies the kth sample as positive}, V_{k}>C)}{V_{k}>C}
\]
The numerator for $\mathrm{SENS}_{\mathrm{MPA}}$ is equal to the following:
\begin{align*}
    \frac{1}{K} &
    [\Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{1}, V_{k}>C)\\
    &+ \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C)\\
    &+ \cdots\\
    ]
\end{align*}
Because it is the case that:
\begin{align*}
\Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C) & \\
= \Pr(T_{1}>V_{k}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C) \\
< \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C) \\
\cdots\\
\Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\varepsilon_{0}+V_{\pi_{2}}\varepsilon_{2}\varepsilon_{0}+\cdots+V_{k-1}\varepsilon_{k-1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C) \\
< \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C) \\
\end{align*}
So, via the above, we have therefore shown that it is the case that the numerator is less than $\Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C)$. 
Thus, we have shown that
\[
\mathrm{SENS}_{\mathrm{MPA}} < \mathrm{SENS}_{\mathrm{MP}}< \mathrm{SENS}_{\mathrm{IND}}
\]
For $\mathrm{SENS}_{\mathrm{mMPA}}$, we have that 

\begin{align*}
\mathrm{SENS}_{\mathrm{mMPA}} &
    = \Pr(\textrm{"mMPA classifies the kth sample as positive"}|V_{k}>C)\\
    & = \frac{\Pr(\textrm{"mMPA classifies the kth sample as positive"}, V_{k}>C)}{\Pr(V_{k}>C)}\\
\end{align*}
The numerator for $\mathrm{SENS}_{\mathrm{mMPA}}$ is 
\begin{align*}
    \frac{1}{K}[\Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{1}=k)\\
+ \Pr(T_{1}>V_{\sigma_{1}}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C|\sigma_{2}=k) \\
+ \cdots \\
+ \Pr(T_{1}>V_{\sigma_{1}}\varepsilon_{1}\varepsilon_{0}+V_{\sigma_{2}}\varepsilon_{2}\varepsilon_{0}+\cdots+V_{\sigma_{k-1}}\varepsilon_{k-1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{K}=k)] \\
\end{align*}
Because it is the case that (upon doing some comparisons): 
\begin{align*}
\Pr(T_{1}>V_{\sigma_{1}}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C|\sigma_{2}=k) \\
< \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{2}=k)\\
\vspace{10 mm}\\
\cdots\\
\vspace{10 mm}\\
\Pr(T_{1}>V_{\sigma_{1}}\varepsilon_{1}\varepsilon_{0}+V_{\sigma_{2}}\varepsilon_{2}\varepsilon_{0}+\cdots+V_{\sigma_{k-1}}\varepsilon_{k-1}\varepsilon_{0}+C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{K}=k) \\
< \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{K}=k)\\
\end{align*}
So, via the above, we have therefore shown that it is the case that the numerator is less than the following:
\begin{align*}
\frac{1}{K}[\Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{1}=k)\\
+ \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C|\sigma_{2}=k)\\
\cdots \\
+ \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C|\sigma_{K}=k) \\
= \Pr(T_{1}>C\varepsilon_{0}, V_{k}>C\varepsilon_{2}, V_{k}>C)
\end{align*}
Thus we have shown that 
\[
\mathrm{SENS}_{\mathrm{mMPA}}<\mathrm{SENS}_{\mathrm{MP}}< \mathrm{SENS}_{\mathrm{IND}}
\]
It remains for us then to prove that it is the case that 
\[
\mathrm{SENS}_{\mathrm{mMPA}}>\mathrm{SENS}_{\mathrm{MPA}}
\]
Since the denominators for $\mathrm{SENS}_{\mathrm{mMPA}}$ and $\mathrm{SENS}_{\mathrm{MPA}}$ are the same. We only need to compare the numerators.
We can compare term-by-term as follows:
\begin{align*}
\Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)\\
< \Pr(T_{1}>C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{1}=k) &\\
\end{align*}   
\begin{align*}
\Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C)  \\
< \Pr(T_{1}>V_{\pi_{1}}\varepsilon_{1}\eta_{1}+C\eta_{1}, V_{k}>C\varepsilon_{k}, V_{k}>C|\sigma_{2}=k) 
\end{align*}
\begin{align*}
    \cdots
\end{align*}
Because the above term-by-term holds true, then we have that 
\[
\mathrm{SENS}_{\mathrm{mMPA}}>\mathrm{SENS}_{\mathrm{MPA}}
\]
Therefore, we have proved that
\[
\mathrm{SENS}_{\mathrm{IND}}>\mathrm{SENS}_{\mathrm{MP}}>\mathrm{SENS}_{\mathrm{mMPA}}>\mathrm{SENS}_{\mathrm{MPA}}
\]
as desired.

\end{proof}

\subsection{Proof of of Theorem 6 Specificity}
\begin{proof}
\begin{align*}
    \mathrm{SPEC}_{\mathrm{POOL}} & 
    = \Pr(\textrm{"sample classified as negative"}|V_{k}<C)\\
    & = \frac{1}{\Pr(V_{k}<C)}\\
\end{align*}
The denominator is very simple, so we shall focus on the numerator.

\begin{align*}
    \mathrm{SPEC}_{\mathrm{IND}} &
    = \frac{1}{\Pr(V_{k}<C)}\Pr(\textrm{"Pooling classifies the kth sample as negative"}, V_{k}<C)\\
    & = \frac{\Pr(V_{k}<C{\varepsilon_{k}}^{-1}, V_{k}<C)}{\Pr(V_{k}<C)}\\
    & = \frac{\Pr(V_{k}<C\varepsilon_{k}, V_{k}<C)}{\Pr(V_{k}<C)}\\
\end{align*}

\begin{align*}
    \mathrm{SPEC}_{\mathrm{MP}} &
    = \frac{\Pr(\textrm{"MP classified the sample as negative"},V_{k}<C)}{\Pr(V_{k}<C)}\\
    & = \frac{\Pr(T_{1}\varepsilon_{0}<C, V_{k}<C) + \Pr(T_{1}\varepsilon_{0}>C, V_{k}\varepsilon_{k}<C, V_{k}<C)}{\Pr(V_{k}<C)}\\
    & = \frac{\Pr(T_{1}<C\varepsilon_{0}, V_{k}<C) + \Pr(T_{1}>C\varepsilon_{0}, V_{k}<C\varepsilon_{k}, V_{k}<C)}{\Pr(V_{k}<C)}\\
\end{align*}

Note
\[
\Pr(T_{1}<C\varepsilon_{0}, V_{k}<C)>\Pr(T_{1}<C\varepsilon_{0}, V_{k}<C\varepsilon_{k}, V_{k}<C)
\]
So
\begin{align*}
    \Pr(T_{1}<C\varepsilon_{0}, V_{k}<C)+\Pr(T_{1}>C\varepsilon_{0}, V_{k}<C\varepsilon_{k}, V_{k}<C) \\
    > \Pr(T_{1}<C\varepsilon_{0}, V_{k}<C\varepsilon_{k}, V_{k}<C)+\Pr(T_{1}>C\varepsilon_{0}, V_{k}<C\varepsilon_{k}, V_{k}<C)\\
    = \Pr(V_{k}<C\varepsilon_{k}, V_{k}<C)\\
\end{align*}
Thus, we have proven that 
\[
\mathrm{SPEC}_{\mathrm{MP}}>\mathrm{SPEC}_{\mathrm{IND}}
\]


\begin{align*}
    \mathrm{SPEC}_{\mathrm{MPA}} &
    = \frac{\Pr(\textrm{"MPA classifies the sample as negative"},V_{k}<C)}{\Pr(V_{k}<C)}\\
\end{align*}

The Numerator is:
\begin{align*}
    \mathrm{A}_{\mathrm{MPA}} &
    = \Pr(T_{1}<C\varepsilon_{0}, V_{k}<C)\\
    & + \Pr(T_{1}<C\varepsilon_{0},V_{k}<C\varepsilon_{1},V_{k}<C|\pi_{1}=k) * \frac{1}{K}\\
    & + \cdots\\
\end{align*}

Note
\begin{align*}
    \Pr(C\varepsilon_{0}<T_{1}<V_\pi_{1}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0},V_{k}<C|\pi_{2}=k) * \frac{1}{K} \\  > \Pr(C\varepsilon_{0}<T_{1}<V_\pi_{1}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0},V_{k}<C\varepsilon_{2},V_{k}<C|\pi_{2}=k) * \frac{1}{K}\\
\end{align*}

So
\begin{align*}
\Pr(C\varepsilon_{0}<T_{1}<V_\pi_{1}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0},V_{k}<C|\pi_{2}=k) * \frac{1}{K} \\   
 + \Pr(T_{1}>V_\pi_{1}\varepsilon_{1}\varepsilon_{0}+C\varepsilon_{0},V_{k}<C\varepsilon_{2}, V_{k}<C|\pi_{2}=k) * \frac{1}{K}\\
 > 
\end{align*}

Similarly,
\begin{align*}
    skdflksdjflkjsdflksdjflksdjflkdsjf
\end{align*} 

Thus we have that,
\begin{align*}
    fjsldkfjldskfjsdlkfjsldkjflsdkfjsldkfjsdlkfj
\end{align*}

So we have proved that 
\[
\mathrm{SPEC}_{\mathrm{MPA}}>\mathrm{SPEC}_{\mathrm{MP}}
\]

\begin{align*}
    \mathrm{SPEC}_{\mathrm{mMPA}} &
    = \frac{\Pr(\textrm{"MPA classifies the sample as negative"},V_{k}<C)}{\Pr(V_{k}<C)}\\
\end{align*}

The Numerator is:
\begin{align*}
    \mathrm{A}_{\mathrm{MPA}} &
    = \Pr(T_{1}<C\varepsilon_{0}, V_{k}<C)\\
    & + \Pr(T_{1}<C\varepsilon_{0},V_{k}<C\varepsilon_{1},V_{k}<C|\pi_{1}=k) * \frac{1}{K}\\
    & + \cdots\\
\end{align*}
You can (similar to MPA) prove that 
\[
\mathrm{SPEC}_{\mathrm{MPA}}>\mathrm{SPEC}_{\mathrm{MP}}
\]

Now we proceed to (attempt to) prove  
\[
\mathrm{SPEC}_{\mathrm{mMPA}}>\mathrm{SPEC}_{\mathrm{MPA}}
\]
Since the denominator is the same, we need only to compare $\mathrm{A}_{\mathrm{mMPA}}$ and $\mathrm{A}_{\mathrm{MPA}}$.

Note:
\begin{align*}
    1 + 1 &
    = 2 \\
    & = 3\\
\end{align*}

Similarly,
\begin{align*}
    
\end{align*}

So 
\begin{align*}
    
\end{align*}

Similarly,
\begin{align*}
    
\end{align*}

We claim that
\begin{align*}
    
\end{align*}
so $\mathrm{A}_{\mathrm{MPA}} < \mathrm{A}_{\mathrm{mMPA}}$. Thus we have $\mathrm{A}_{\mathrm{MPA}} < \mathrm{A}_{\mathrm{mMPA}}$
\end{proof}



==> proof_of_corollary4.tex <==
 
